BDFA: A Blind Data Adversarial Bit-flip Attack on Deep Neural Networks

Adversarial bit-flip attack (BFA) on Neural Network weights can result in catastrophic accuracy degradation by flipping a very small number of bits. A major drawback of prior bit flip attack techniques is their reliance on test data. This is frequently not possible for applications that contain sensitive or proprietary data. In this paper, we propose Blind Data Adversarial Bit-flip Attack (BDFA), a novel technique to enable BFA without any access to the training or testing data. This is achieved by optimizing for a synthetic dataset, which is engineered to match the statistics of batch normalization across different layers of the network and the targeted label. Experimental results show that BDFA could decrease the accuracy of ResNet50 significantly from 75.96\% to 13.94\% with only 4 bits flips.

==> Prim.tex <==
% %\section{An Adversarial Attack via Input/Weight Perturbation}

% \section{Preliminaries}

% \subsection{Attack Assumptions}
% In this paper, we assume that we have access to DNN parameters and architecture. 
% We can effectively attack any Deep learning model with batch normalization layers.
% However, unlike previous works, we do not have access to any training/test data. 

% \subsection{Deep Learning Datasets}

% In supervised learning, particularly computer vision tasks (image classification[], object detection[], etc.), we have some training data D that contains data points $(x,y)$, where $(x,y)$ are drawn from an unknown distribution P.

% \begin{equation}
%     D = \{(x_1,y_1),(x_2,y_2),...,(x_n,y_n)\}
% \end{equation}

% By the help of a Neural network, we train a function H on D, so that we can predict $H(x)=y$ with a high probability where $(x,y) \sim P$ is a new data point that was not in $D$. We can achieve this goal by minimizing a loss function L (e.g. Cross Entropy [], Mean Squared Error [], etc.) on D, through adjusting DNN parameters.
% % \begin{equation}
% %     Minimize \quad \frac{1}{n} \sum \mathcal{L}(H(x),y)
% % \end{equation}
% \begin{equation}
%     Minimize \mathcal{L} = \frac{1}{N} \sum^{N}_{i=1} \;\;\mathclap{f}\;( H(X_{i};B) , Y_i)
% \end{equation}
% % \subsection{BFA}
% % Bit-Flip Attack (BFA) \cite{rakin2019bit} uses a batch of training data inputs to find the most vulnerable bit, which is the bit with the highest gradient on the loss function L, and flips it. By repeating this process for a few times, BFA is able to drastically decrease the accuracy of the DNN model.
